Effects of Automated Interventions in Programming Assignments: Evidence from a Field Experiment

A typical problem in MOOCs is the missing opportunity for course conductors to individually support students in overcoming their problems and misconceptions. This paper presents the results of automatically intervening on struggling students during programming exercises and offering peer feedback and tailored bonus exercises. To improve learning success, we do not want to abolish instructionally desired trial and error but reduce extensive struggle and demotivation. Therefore, we developed adaptive automatic just-in-time interventions to encourage students to ask for help if they require considerably more than average working time to solve an exercise. Additionally, we offered students bonus exercises tailored for their individual weaknesses. The approach was evaluated within a live course with over 5,000 active students via a survey and metrics gathered alongside. Results show that we can increase the call outs for help by up to 66% and lower the dwelling time until issuing action. Learnings from the experiments can further be used to pinpoint course material to be improved and tailor content to be audience specific.

==> sections/implementation.tex <==
%!TEX root = ../interventions.tex

%\section{Implementation}
%We will focus on the relevant implementation details here that are beneficial for understanding the experiment outcomes.
%Considering the bonus exercises, all important details have already been explained in the concept section.
%\subsection{Architecture}





%\subsection{Bonus Exercises} \label{subsec:implBonusExercises}
%Here we just implemented the workflows which were described in detail in the concept section.


==> sections/problem_statement.tex <==
%!TEX root = ../cluster.tex

\section{Problem Statement}
